Optimal Mini-Batch Size Selection for Fast Gradient Descent

This paper presents a methodology for selecting the mini-batch size that minimizes Stochastic Gradient Descent (SGD) learning time for single and multiple learner problems. By decoupling algorithmic analysis issues from hardware and software implementation details, we reveal a robust empirical inverse law between mini-batch size and the average number of SGD updates required to converge to a specified error threshold. Combining this empirical inverse law with measured system performance, we create an accurate, closed-form model of average training time and show how this model can be used to identify quantifiable implications for both algorithmic and hardware aspects of machine learning. We demonstrate the inverse law empirically, on both image recognition (MNIST, CIFAR10 and CIFAR100) and machine translation (Europarl) tasks, and provide a theoretic justification via proving a novel bound on mini-batch SGD training.

==> Sections/ComparisonConvergenceRate.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparison to Convergence Rate of Gradient Descent Method}

Note that Eqn.~\ref{eqn:PowerDenom} appears to suggest exponential convergence because of the power of $k$ term in the denominator. A closer
analysis shows that this is not correct. Specifically, in the limit
$\sigma \rightarrow 0$, the well-known $1/k$ convergence rate of
gradient descent is recovered:
\begin{equation}
\Delta_{k} \leq {\frac{2\sigma}{\left( 1 + 2\lambda\sigma k + \cdots \right)\left( \frac{2\sigma}{\Delta_{0} - \sigma} + 1 \right)\  - 1} + \sigma} = \frac{1}{\frac{1}{\Delta_{0}} + \lambda k}.
\end{equation}
Also, one can show that the bound is always bigger than the limit:
\[\text{\ \ }\frac{1}{\left( 1 + 2\lambda\sigma \right)^{k}\left( \frac{1}{\Delta_{0} - \sigma} + \frac{1}{2\sigma} \right)\  - \frac{1}{2\sigma}} + \sigma \geq \frac{1}{\frac{1}{\Delta_{0}} + \lambda k},\]
and thus, the exponential term cannot converge faster than $1/k$. The proof follows from expanding $\left( 1 + 2\lambda\sigma \right)^{k}$
to the first order and simplifying, and using
$\Delta_{0} \geq \sigma.$


==> Sections/PracticalConsiderations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Practical Considerations: Estimating
$\mathbf{N_{\infty}}$ and $\mathbf{\alpha}$\label{sec:Estimation}}

In order to exploit the inverse relationship for efficient system
design, one needs to estimate $\alpha$ and $N_{\infty}$ from an
empirical $\NU$ curve, and do so in a
computationally efficient way. This goal can be achieved by evaluating
$\NU$ at two values of $M$ and averaging
as needed to remove noise from random initialization, SGD, etc. If the
values of M are chosen strategically, the overhead of measuring
$\alpha$ and $N_{\infty}$ can be reduced. And in practice, as one
explores a learning model, many experiments are run. So, the cost of
estimating $\alpha$ and $N_{\infty}$ is amortized.

One must of course recognize that when significant changes are made to
the learning task (e.g., major topology change, learning rate change,
target loss change, etc.) $\alpha$ and $N_{\infty}$ might need to be
re-estimated. Thus, looking for other ways to further improve efficiency
is an important research direction.

Our theoretical analysis suggests another path forward: Section~\ref{sec:Theory}
suggests that $N_{\infty}$ behaves like a constant $+1/\epsilon$. Inspired by
that result, we fit $\alpha$ and $N_{\infty}$ for various values of the
training loss, $\epsilon$. From the corresponding plots shown in Figure~\ref{fig:EpsilonDependence}, one
can see that the fits are very good for small $\epsilon$ but grown noisier as $\epsilon$
grows. This relationship might be due to early stopping from large $\epsilon$
leading to lots of very different solutions.
\begin{figure}[ht]
  \centering
  \includegraphics[width=5.99306in,height=3.24792in]{Figures/EpsilonDependence.png}
  \caption{$N_{\infty}$ and $\alpha$ with various $\epsilon$ for the
CIFAR10 dataset for a constant learning rate.}
  \label{fig:EpsilonDependence}
\end{figure}

We then plotted $\alpha$ and $N_{\infty}$ versus $\epsilon$ in Figure~\ref{fig:NAvsEpsilon}, from
which one can see that both exhibit a $1/\epsilon$ relationship for small $\epsilon$. If
this relation holds in general, then one could estimate $\alpha$ and
$N_{\infty}$ once for a given $\epsilon$ and then use the $1/\epsilon$ relationship to
calculate update $\alpha$ and $N_{\infty}$ for other values of $\epsilon$. However, these preliminary results need further study.
\begin{figure}[ht]
  \centering
  \includegraphics[width=2.75774in,height=2.37778in]{Figures/NAvsEpsilon.png}
  \caption{$N_{\infty}$ and $\alpha$ versus $\epsilon$ in blue and
red, respectively, and $1/\epsilon$ fits shown as dashed lines. Both
$N_{\infty}$ and $\alpha$ exhibit a $1/\epsilon$ relationship.}
  \label{fig:NAvsEpsilon}
\end{figure}
